First Results for the pLGAD Sensor for Low-Penetrating Particles

Silicon sensors are the go-to technology for high-precision sensors in particle physics. But only recently low-noise silicon sensors with internal amplification became available. The so-called Low Gain Avalanche Detector (LGAD) sensors have been developed for applications in High Energy Physics, but lack two characteristics needed for the measurement of low-energy protons (<60 keV): a thin entrance window (in the order of tens of nm) and the efficient amplification of signals created near the sensor's surface (in a depth below 1 um). In this paper we present the so-called proton Low Gain Avalanche Detector (pLGAD) sensor concept and some results from characterization of the first prototypes of the sensor. The pLGAD is specifically designed to detect low-energy protons, and other low-penetrating particles. It will have a higher detection efficiency than non-silicon technologies, and promises to be a lot cheaper and easier to operate than competing silicon technologies.

==> content/active-edge.tex <==
Active edge blabla

\begin{figure}[htb]
	\centering
		\includegraphics[width=\textwidth]{figs/pLGAD + active edge.pdf}
	\caption{pLGAD with active edge}	
	\label{fig:plgad_active_edge}
\end{figure}


==> content/elad.tex <==
\gls{ELAD} blabla

\begin{figure}[htb]
	\centering
		\includegraphics[width=\textwidth]{figs/pLGAD + ELAD.pdf}
	\caption{pLGAD with ELAD structure}	
	\label{fig:plgad_elad}
\end{figure}

\begin{figure}[htb]
	\centering
		\includegraphics[width=\textwidth]{figs/pLGAD + active edge + ELAD.pdf}
	\caption{pLGAD with active edge and ELAD structure}	
	\label{fig:plgad_active_edge_elad}
\end{figure}


==> content/performance.tex <==
%---------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Data acquisition requirements}
\label{sec:daq_requirements}

In principle, a pLGAD sensor can be read out with similar readout systems as other \gls*{planar} sensors.
But in contrast to HEP, the investigated particles do not cross the sensor, and leave only a tiny signal.
This leads to the following requirements for the DAQ system:
\begin{itemize}
	\item{self-triggering:}
		In many low-energy physics experiments, the events do not have a defined time structure, where the readout is triggered by an external trigger signal.
		Instead, the DAQ system has to be self-triggering (or ``data-driven'').
	\item{low noise:}
		While the pLGAD sensor increases the SNR by design, a low-noise DAQ system still plays an important role in achieving a high detection efficiency.
	\item{charge sensitive:} 
		Depending on the application, the DAQ system may need to record the signal height - i.e., the charge deposited in the sensor - and not only register a binary hit.
		That way - depending on the deposited charge of the involved particles - one can perform spectroscopic measurements
		%		\footnote{It would be desirable to record the exact pulse shape (see \cref{sec:simulation}), because with that information background rejection could be performed with higher accuracy.
%		However, that is quite a challenge, given the short pulse duration and small amplitude.}
		and identify background events.
	\item{multi-channel:}
		In order to keep the noise in check, each sensing element should be small (see also \cref{sec:noise}.)
		Consequently, when an application requires a large area sensor, the total active area has to be divided into multiple sensing elements.
		This also allows for position-sensitive measurements, e.g., in the form of a hybrid pixel sensor.
\end{itemize}

%---------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Noise estimation}
\label{sec:noise}

For the noise estimation of the pLGAD concept, we take a closer look at three combinations of sensor layouts and readout electronics (for specifications see \cref{tab:noise_parameters}):
\begin{enumerate}
	\item{Single channel prototypes with AliVata~\cite{alivata} readout:} 
		Simple, small sensor with one unstructured electrode.
		This electrode is connected to one channel of the AliVata's VATAGP7 chip~\cite{vatagp7} with a wire bond.
	\item{Pixelated sensor with NoMoS layout and Timepix3~\cite{timepix3} readout:} 
		The sensor is optimized to match the specifications of the NoMoS measurement concept, with $256 \times 32$ pixels of size $0.4\times\SI{1.6}{\milli\meter}^2$ and a thickness of \SI{1}{\milli\metre}. 
		The pixels are routed to the inputs of the Timepix3 chip in a second metal layer.
	\item{Pixelated sensor with Timepix3 native layout:} 
		Hybrid pixel sensor whose pixel layout matches the input channel grid of the Timepix3 chip. 
		No additional routing lines are needed.
\end{enumerate}

\begin{table*}[htb]

\centering
	\begin{tabular}{rlll}
		\toprule
		Parameter & Single channel & NoMoS & Timepix3 native \\
		\midrule
		Capacitive noise $\ENC_\mathrm{C}$ 			& 192.6 	& 62.0\hphantom{0} 			& 62.0\hphantom{0}  \\
		Leakage current noise $\ENC_\mathrm{J}$	& 148.1 	& 63.5 		& \hphantom{0}2.5 \\
		Parallel resistor noise ${\ENC}_{\RP}$ 	& \hphantom{0}17.3 		& 17.26 	& 17.3 \\
		Series resistor noise ${\ENC}_{\RS}$ 		& \hphantom{0}19.7 		& \hphantom{0}0.37 		& \hphantom{0}0.01 \\
		\midrule
		Quadratic sum $\ENC$ 													& 244.4 	& 90.4		& 64.4 \\
		Detection threshold	$p_\mathrm{min}$	& 123 & 46 & 33 \\
		\bottomrule
	\end{tabular}
	\caption{Equivalent Noise Charge (ENC) contributions for three variants of pLGAD detection systems, all values are in \glspl{electron}.
	Note that the Timepix3 chip has a self-triggering threshold of 500 \glspl{electron}~\cite{timepix3_2014}, so the detection thresholds calculated here can only be achieved with external triggering. Due to this, for experiments that can not have external triggering, such as NoMoS, the detection threshold is limited to above 50 \glspl{electron}, assuming a gain of 10 and a pLGAD connected to a self-triggered Timepix3 chip.}
	\label{tab:noise_contributions}
\end{table*}
With the assumptions, specifications, and the equations presented in \ref{sec:noise_calculation}, the Equivalent Noise Charge (ENC) contributions result in the noise estimates listed in \cref{tab:noise_contributions}.
Note that these values are best-case approximations.
The detection threshold values promise very good performance for low-penetrating particles, as is also shown in \cref{sec:technologies}.
Of course, to fully exploit a pLGAD sensor's potential, more effort has to go into the design of the DAQ system, especially in order to minimize external noise sources stemming from the DAQ system.

\begin{figure*}[tb]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=0.8\textwidth]{figs/DEPFET-principle.png}
		\caption{The DEPFET sensor integrates the first stage of the readout electronics into the sensor. The signal \glspl{electron} are stored in a potential minimum (the \gls*{internal gate}), and can be read repeatedly~\cite{Kemmer1987}. Image courtesy of L. Andricek~\cite{depfet_drawing}}	
		\label{fig:depfet}
	\end{subfigure}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=0.8\textwidth]{figs/silicon-drift-detector-features-n.png}
		\caption{The SDD sensor uses an electrical \gls*{drift} field to guide the signal charge towards a central field effect transistor~\cite{Gatti1984}.}	
		\label{fig:sdd}
	\end{subfigure}
	\caption{Competing sensor technologies.}
	\label{fig:alternatives}
\end{figure*}


\subsection{Comparison to competing technologies}
\label{sec:technologies}

The pLGAD sensor fills a gap where only two other technologies have comparable properties: DEPFET and SDD.
DEPFET sensors are produced at the MPG HLL~\cite{HLL} (The Halbleiterlabor of the Max Planck Society) and at PNSensor~\cite{pnsensor}, while SDDs are, apart from MPG HLL and PNSensor, also manufactured at FBK-CMM~\cite{fbk} (Fondazione Bruno Kessler – Center for Materials and Microsistems).
Both the DEPFET technology~\cite{Kemmer1987} (\cref{fig:depfet}) and the SDD technology~\cite{Gatti1984} (\cref{fig:sdd}) are well-established and versatile, can be operated in a fully-depleted state, and allow for back-illumination (unstructured entrance window for impinging particles) with a very thin entrance window in the order of 10s of nms.
%But these alternatives come at a price.


\begin{figure*}[htb!]
	\centering
	\includegraphics[width=\textwidth]{figs/ProtonDetectionRateImsil.png}
	\caption{Detection efficiency of \glspl{proton} with different energies at normal incidence, as a function of the detection threshold of the DAQ system in \glspl{electron}. The efficiency calculation is based on an IMSIL simulation of 50,000 protons impinging on a silicon sensor with a \SI{15}{\nano\meter} thick, non-active aluminium entrance window, and uses the best case CCE shown in \cref{fig:entrance_window} top.
		%\Glspl{proton} can go undetected due to \gls*{backscattering}, when they deposit too little energy in the active region of the sensor, or when they are completely stopped in the non-active layer.
		The expected detection thresholds of pLGAD and {DEPFET} sensors are indicated as vertical lines.
		The most likely operating point of the NoMoS measurement concept is highlighted with a circle.
		Details on the simulation can be found in \ref{sec:detection_efficiency}.}	
	\label{fig:detection_rate}
\end{figure*}


During the research for viable sensors, we asked for the possible performance of a DEPFET sensor with the pixel layout needed for the NoMoS measurement concept (cf. \cref{sec:noise}), which was kindly provided by HLL~\cite{Lechner_private}.
With that information we can directly compare the performance of the pLGAD and the DEPFET sensors in \cref{fig:detection_rate}.
A DEPFET sensor with appropriate pixel geometry reaches a detection threshold of below 30 \glspl{electron}, if cooled to \SI{-50}{\celsius}. Alternatively, DEPFET sensors have been shown to be able to detect single signal \glspl{electron} by using correlated double-sampling (to do pedestal subtraction in-situ) and repetitive non-destructive readout (to reduce noise)~\cite{baehr2017}. However, these methods take time and therefore limit the rate capability of the sensor, which is unfeasible for the NoMoS measurement concept.
The pLGAD system is limited to above 50 \glspl{electron} at room temperature, by assuming it has a gain of 10 and is connected to a self-triggered Timepix3 chip. (see \cref{tab:noise_contributions})

Both DEPFET and SDD technologies introduce a number of complications: the sensors are intricate, and therefore expensive, and require at least 7 (5 for SDD) different operation voltages.
For a DEPFET sensor, cooling is mandatory to keep the \gls*{leakage current} and its corresponding noise low, and thus increase the \gls*{detection efficiency} (cf. \cref{fig:detection_rate}).
In addition, the DEPFET technology involves several different custom readout chips, and has a relatively low frame rate, compared to some other planar silicon sensors, in the order of microseconds~\cite{valentan2016}.

\noindent In contrast to DEPFET and SDD, the proposed pLGAD sensor 
\begin{itemize}
	\item{is a lot cheaper, because of the simple \gls*{planar} production process}
	\item{works with commercial readout systems that can read \gls*{planar} sensors}
	\item{can be operated with only one supply voltage}
	\item{can be operated at room temperature}
	\item{has a very high intrinsic time resolution}

\end{itemize}


\cref{fig:detection_rate} shows the \gls*{proton} detection efficiency as a function of the detection threshold of the DAQ system, for different \gls*{proton} energies at normal incidence (details on the simulation can be found in \ref{sec:detection_efficiency}).
\Glspl{proton} can go undetected due to \gls*{backscattering}, when they deposit too little energy in the active region of the sensor, or when they are completely stopped in the \gls*{entrance window}.
For \SI{15}{\kilo\eV} (the minimum \gls*{proton} energy in NoMoS after the most likely post-acceleration), the pLGAD sensor outperforms an uncooled DEPFET sensor with the same pixel layout, and achieves almost the same detection efficiency as a cooled one.
A proton loss in the order of 0.15\% (or a detection efficiency of 99.85\%) seems feasible, as a best case scenario, due to convolution of CCE (cf. \cref{fig:entrance_window}). It should be noted that the curves presented in \cref{fig:detection_rate} are valid for \SI{15}{\kilo\eV} \glspl{proton}. For NoMoS, the protons will range from \SIrange{15}{15.8}{\kilo\eV} after post-acceleration.



%\subsection{Proton energy range}
%\label{sec:energy_range}

==> content/variants.tex <==
Variants blabla

\subsection{Active edge: Optimization of the electric field outside of the sensor}
\label{sec:active_edge}

\begin{figure}[htb]
	\centering
		\includegraphics[width=\textwidth]{figs/pLGAD + active edge.pdf}
	\caption{pLGAD with active edge}	
	\label{fig:plgad_active_edge}
\end{figure}


\subsection{Enhanced lateral drift: Optimization of the position resolution}
\label{sec:elad}

\gls{ELAD} blabla

\begin{figure}[htb]
	\centering
		\includegraphics[width=\textwidth]{figs/pLGAD + ELAD.pdf}
	\caption{pLGAD with ELAD structure}	
	\label{fig:plgad_elad}
\end{figure}

\subsection{Material sandwich: Optimization of stopping power}
\label{sec:bonding}


==> glossary_ignored.tex <==
% Special glossary for ignored entries.
\newignoredglossary{ignored}
%Use \glsmoveentry{<key>}{ignored} to move an entry from the regular glossary to the ignored one
%Hyperlinking for these entries is disabled.
\glsmoveentry{electron}{ignored}
\glsmoveentry{proton}{ignored}
\glsmoveentry{neutrino}{ignored}
\glsmoveentry{generation}{ignored}
\glsmoveentry{quark}{ignored}
\glsmoveentry{lepton}{ignored}
\glsmoveentry{hadron}{ignored}
\glsmoveentry{boson}{ignored}
\glsmoveentry{fermion}{ignored}
\glsmoveentry{intrinsic}{ignored}
\glsmoveentry{extrinsic}{ignored}
\glsmoveentry{gauge theory}{ignored}
\glsmoveentry{gravitation}{ignored}
\glsmoveentry{Hamiltonian}{ignored}
\glsmoveentry{hierarchy problem}{ignored}
\glsmoveentry{Lagrangian}{ignored}
\glsmoveentry{Lie group}{ignored}
\glsmoveentry{neutron}{ignored}
\glsmoveentry{perturbation theory}{ignored}
\glsmoveentry{photon}{ignored}
\glsmoveentry{positron}{ignored}
\glsmoveentry{strong}{ignored}
\glsmoveentry{supersymmetry}{ignored}
\glsmoveentry{weak}{ignored}
\glsmoveentry{bulk}{ignored}
\glsmoveentry{photo resist}{ignored}
\glsmoveentry{wafer}{ignored}
\glsmoveentry{Standard Model}{ignored}
\glsmoveentry{doping}{ignored}
\glsmoveentry{dopant}{ignored}
\glsmoveentry{donor}{ignored}
\glsmoveentry{acceptor}{ignored}
\glsmoveentry{implantation}{ignored}
\glsmoveentry{n-type}{ignored}
\glsmoveentry{p-type}{ignored}
\glsmoveentry{pnjunction}{ignored}
\glsmoveentry{hole}{ignored}

